Generating Semantic Graph Corpora with Graph Expansion Grammar

We introduce Lovelace, a tool for creating corpora of semantic graphs. The system uses graph expansion grammar as a representational language, thus allowing users to craft a grammar that describes a corpus with desired properties. When given such grammar as input, the system generates a set of output graphs that are well-formed according to the grammar, i.e., a graph bank. The generation process can be controlled via a number of configurable parameters that allow the user to, for example, specify a range of desired output graph sizes. Central use cases are the creation of synthetic data to augment existing corpora, and as a pedagogical tool for teaching formal language theory.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{Rudolf Freund, Benedek Nagy (Eds.): 13th International Workshop on \\ Non-Classical Models of Automata and Applications (NCMA 2023)\\
EPTCS 388, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.388.3}{10.4204/EPTCS.388.3}}


==> fig-graph.tex <==
     \node at (1,1.5) [overtex, label=above:\prt 1] (x1) {\footnotesize $b$};
     \node at (4.75,1.5) [overtex, label=above:\prt 2] (x2) {\footnotesize $a$};
     \node at (7,1.5) [overtex, label=above:\prt 4] (x3) {\footnotesize $b$};
     
     \node at (0,0) [overtex, label=below:\dk 1] (y1) {};
     \node at (2,0) [overtex] (y2) {\footnotesize $c$};
     \node at (4,0) [overtex] (y3) {\footnotesize $b$};
     \node at (6,0) [overtex, label=above right:\prt 3, label=below:{\dk 2,\,\dk 3}] (y4) {};
     
    %  \node at (5.5,-1.25) (note) {\footnotesize Neither in \emph{ports} nor in \emph{dock} ( ``context node")};
     %    \draw[->,-latex,dashed,bend left=20] (note.west) to (y2);
     
    \draw[->,line width=0.30mm,-latex,bend left=7] (x1) to (x2);
    \draw[->,line width=0.30mm,-latex,bend right=10] (x1) to (y1);
    \draw[->,line width=0.30mm,-latex,bend left=10] (x1) to  (y2) ;
    \draw[->,line width=0.30mm,-latex,bend right=10] (x2) to (y2);
    \draw[->,line width=0.30mm,-latex,bend right=5] (x2) to (y3);
    \draw[->,line width=0.30mm,-latex,bend left=10] (x2) to (y4);
    
        
  
